On the Almost Sure Convergence of Stochastic Gradient Descent in Non-Convex Problems

This paper analyzes the trajectories of stochastic gradient descent (SGD) to help understand the algorithm's convergence properties in non-convex problems. We first show that the sequence of iterates generated by SGD remains bounded and converges with probability $1$ under a very broad range of step-size schedules. Subsequently, going beyond existing positive probability guarantees, we show that SGD avoids strict saddle points/manifolds with probability $1$ for the entire spectrum of step-size policies considered. Finally, we prove that the algorithm's rate of convergence to Hurwicz minimizers is $\mathcal{O}(1/n^{p})$ if the method is employed with a $\Theta(1/n^p)$ step-size schedule. This provides an important guideline for tuning the algorithm's step-size as it suggests that a cool-down phase with a vanishing step-size could lead to faster convergence; we demonstrate this heuristic using ResNet architectures on CIFAR.

==> App-Erratum.tex <==
%----------------------------------------------------------------------
%%% APP: ERRATUM
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


There was a typo on Lines 60 and 258 of the body of our paper:
the definition of a hyperbolic equilibrium point involves the condition $\det\nabla^{2}\obj(\sol) \neq 0$, not $\nabla^{2}\obj(\sol) \ml 0$.
This typo has been corrected herein.

==> Impact.tex <==
%----------------------------------------------------------------------
%%% IMPACT
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This work does not present any foreseeable societal consequence.

==> Rates.tex <==
%----------------------------------------------------------------------
%%% RATES
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


We conclude our analysis of \eqref{eq:SGD} by examining the algorithm's rate of convergence.
Because we are primarily interested in the convergence of the algorithm's trajectories, we focus here on the distance $\curr[\breg] = (1/2) \norm{\curr - \sol}^{2}$ between the iterates of \eqref{eq:SGD} and a local minimizer of $\obj$.%

Given that any convergence rate analysis of this type must be necessarily local (as $\obj$ is non-convex), we will examine the algorithm's convergence to local minimizers $\sol\in\sols$ that are regular in the sense of Hurwicz, \ie $\hmat(\sol) \mg 0$.
Our main result in this regard is the following.

\begin{restatable}{theorem}{rate}
\label{thm:rate}
Fix some tolerance level $\delta>0$,
let $\sol$ be a regular minimizer of $\obj$,
and
suppose that \cref{asm:noise} holds.
Assume further that \eqref{eq:SGD} is run with a step-size schedule of the form $\curr[\step] = \step/(\run + \offset)^{\pexp}$ for some $\pexp \in (2/(\qexp + 2),1]$ and large enough $\offset,\step > 0$.
Then:
\begin{enumerate}
\setlength{\itemsep}{\smallskipamount}
\item
There exist neighborhoods $\nhd$ and $\nhd_{1}$ of $\sol$ such that, if $\init\in\nhd_{1}$, the event
\begin{equation}
\label{eq:stay}
\event_{\nhd}
	= \{\curr\in\nhd\;\text{for all $\run=\running$}\}
\end{equation}
occurs with probability at least $1-\delta$.
\item
Conditioned on $\event_{\nhd}$, we have
\begin{equation}
\label{eq:rate}
\exof{\norm{\curr - \sol}^{2} \given \event_{\nhd}}
	 = \bigoh(1/\run^{\pexp}).
\end{equation}
\end{enumerate}
\end{restatable}


%----------------------------------------------------------------------
%% Rates figure begins here

\begin{figure*}[t]
\centering
\footnotesize
\includegraphics[width=6.25cm]{Figures/RastriginFull.pdf}%
\hfill
\includegraphics[width=6.25cm]{Figures/RastriginFull-d50T10E3.pdf}%
%\begin{subfigure}{.45\linewidth}
%\includegraphics[width=.9\columnwidth]{Figures/RastriginFull.pdf}%
%%\caption{Some subcaption}
%\end{subfigure}
%\hfill
%\begin{subfigure}{.45\linewidth}
%\includegraphics[width=.9\columnwidth]{Figures/RastriginFull-d50T10E3.pdf}%
%%\caption{Some subcaption}
%\end{subfigure}
\caption
[Some caption]
{The rate of convergence of \eqref{eq:SGD} in the Rastrigin risk benchmark $\obj(\point) = \sum_{i=1}^{\vdim} \bracks{\point_{i}^{2} - \cos(2\pi\point_{i})}$ with $\vdim=50$ and $\vdim=500$ degrees of freedom (left and right respectively).
In both cases, we ran $N=10^{3}$ instances of \eqref{eq:SGD} with a $1/\run$ and a $1/\sqrt{\run}$ step-size schedule and the same seeds across schedules.
Each plot depicts the value difference $\obj(\curr) - \obj_{\infty}$ for a sample run, the sample average (marked black line), and the min-max spread of the samples (shaded blue and red for the $1/\run$ and $1/\sqrt{\run}$ policies respectively).
The $1/\run$ schedule outperforms $1/\sqrt{\run}$ by $2$ to $4$ orders of magnitude, and the difference becomes more pronounced in higher-dimensional problems.}
%\vspace{-2ex}
\label{fig:rates}
\end{figure*}
%% Rates figure ends here
%----------------------------------------------------------------------


We should note here that \cref{thm:rate} does not presuppose \cref{asm:reg,asm:sublvl,asm:gradlvl};
since the rate analysis is local, the differentiability of $\obj$ suffices.
On that account, the guarantee \eqref{eq:rate} immediately translates into a value convergence rate by bounding $\obj(\curr) - \obj(\sol)$ from above by $\norm{\curr-\sol}^{2}$.
For this reason, we do not distinguish between value \vs mean square convergence;
we illustrate this in \cref{fig:rates} where we plot the value convergence rate of \eqref{eq:SGD}.
%in a standard non-convex benchmark function.

The proof of \cref{thm:rate} relies on the observation that, if $\curr$ is near a regular minimizer $\sol$, we have the bound
\begin{equation}
\label{eq:bound-loc}
\next[\breg]
	\leq (1 - \qmin\curr[\step]) \curr[\breg]
	+ \curr[\step]\curr[\snoise]
	+ \tfrac{1}{2} \curr[\step]^{2} \norm{\curr[\signal]}^{2},
\end{equation}
where $\curr[\snoise]$ is a martingale noise term and $\qmin>0$ is a constant that depends on $\lambda_{\min}(\hmat(\sol))$ and $\nhd$.
If this bound held globally, taking expectations would eliminate the noise term and allow us to employ numerical analysis arguments to obtain the decay rate of $\exof{\curr[\breg]}$.
However, since a \emph{single} bad realization of the noise can throw the algorithm out of the region of validity of \eqref{eq:bound-loc}, it is not possible to do so.
Instead, we first show that $\sol$ is \emph{stochastically stable}, \ie with high probability, any initialization that is close enough to $\sol$ remains close enough.
Conditioning on this event, \eqref{eq:bound-loc} is guaranteed to hold;
however, this conditioning also changes the statistics of the noise term $\curr[\snoise]$,
\emph{which is no longer unbiased after conditioning}.
Overcoming this difficulty requires an intricate probablistic argument that we present in the supplement (where we also provide explicit expressions of the constants in the estimate of \cref{thm:rate}).

==> SA-old.tex <==
%----------------------------------------------------------------------
%%% STOCHASTIC APPROXIMATION
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


%----------------------------------------------------------------------
%%% GRADIENT FLOWS
%----------------------------------------------------------------------
\subsection{Gradient descent in continuous time}
\label{sec:GD}

Our point of departure will be to recast \eqref{eq:SGD} as
\begin{equation}
\frac{\next - \curr}{\curr[\step]}
%	= \curr[\signal]
	= \nabla(\obj(\curr)) + \curr[\noise].
\end{equation}
Written this way, $\curr$ can be seen as a \acl{RM} discretization of the continuous-time \acli{GD}
\begin{equation}
\label{eq:GD}
\tag{GD}
\dorbit{\ctime}
	= - \nabla\obj(\orbit{\ctime}).
\end{equation}
A key point of making this comparison with \eqref{eq:GD} is that
\begin{equation}
\label{eq:Lyapunov}
\frac{d\obj}{dt}
%\ddt\obj(\orbit{\ctime})
	= \braket{\nabla\obj(\orbit{\ctime})}{\orbit{\ctime}}
	= - \dnorm{\nabla\obj(\orbit{\ctime})}^{2}
	\leq 0,
\end{equation}
with equality if and only if $\nabla\obj(\orbit{\ctime}) = 0$ (\ie if and only if $\orbit{\ctime} \in \sols$).
In turn, this \emph{strict Lyapunov} property leads to the following strong convergence result:

\begin{proposition}
[Gradient flow convergence]
\label{prop:conv-GD}
Under \cref{asm:reg,asm:sublvl}, every solution $\orbit{\ctime}$ of \eqref{eq:GD} converges to $\sols$.
\end{proposition}

The ``vanilla'' statement of this result is that any invariant set of limit points of \eqref{eq:GD} is contained in $\sols$ \textendash\ see \eg \citet[Prop.~6.4]{Ben99} or \citet[p.~118]{Bor08}.
\Cref{prop:conv-GD} is slightly stronger in that regard because it actually implies convergence to $\sols$ (\ie $\orbit{\ctime}$ does not escape to infinity);
for completeness, we provide a proof in the paper's supplement.


%----------------------------------------------------------------------
%%% APT
%----------------------------------------------------------------------
\para{Asymptotic pseudotrajectories}
%\label{sec:APT}

In view of \cref{prop:conv-GD}, if the trajectories of \eqref{eq:SGD} are ``good enough'' approximations of the solution trajectories of \eqref{eq:GD}, one would expect \eqref{eq:SGD} to enjoy similar convergence properties.
{This idea is the lodestar of our analysis;}
to make it precise, we will need to properly define the following:
%\vspace{-\smallskipamount}
\begin{enumerate}
%[\upshape(\itshape i\upshape)]
\setlength{\itemsep}{\smallskipamount}
\item
A ``continuous-time'' version of the sequence $\curr$.
\item
A measure of ``closeness'' between this continuous trajectory and the solution orbits of \eqref{eq:GD}.
\end{enumerate}
%\vspace{-\smallskipamount}

For the first, a natural way to proceed is to view each $\curr[\step]$ as a ``forward time-step'' and introduce the \emph{proper time} variable
%\begin{equation}
%\label{eq:proper}
%\txs
%\curr[\proper]
%	= \sum_{\runalt=\start}^{\run-1} \iter[\step],
%\end{equation}
\begin{equation}
\label{eq:proper}
%\txs
\curr[\proper]
	= \sum\nolimits_{\runalt=\start}^{\run} \iter[\step].
\end{equation}
%with $\proper_{0} = 0$ (by the empty sum convention).
Informally, $\curr[\proper]$ represents the elapsed time at the $\run$-th iteration of \eqref{eq:SGD}, so the continuous-time interpolation of $\curr$ can be defined as $\apt{\ctime} = \init$ for $\ctime\in[0,\init[\proper]]$ and
\begin{equation}
\label{eq:interpolation}
\apt{\ctime}
	= \curr
		+ \frac{\ctime - \curr[\proper]}{\next[\proper] - \curr[\proper]} (\next - \curr)
\end{equation}
for all $\ctime \in [\curr[\proper],\next[\proper]]$, $\run\geq\start$.
%and
%$\apt{\ctime} = \init$ for $\ctime\in[0,\init[\proper]]$.

For the second, one should first note that comparing $\apt{\ctime}$ to a \emph{fixed} solution trajectory $\orbit{\ctime}$ of \eqref{eq:GD} is not meaningful;
instead,
%because of the noise in \eqref{eq:SGD},
any comparison between $\apt{\ctime}$ and \eqref{eq:GD} should involve an \emph{ensemble} of such solutions.
On that account, it will be convenient to introduce the (negative) \acli{GF} of $\obj$ as the map $\flowmap\from\R_{+}\times\points\to\points$ which, for all $\ctime\in\R_{+}$, sends a point $\point\in\points$ to the point $\flow{\ctime}{\point}\in\points$ obtained by following for time $\ctime$ the solution of \eqref{eq:GD} starting at $\point$.%
\footnote{In words, the curve $\flow{\ctime}{\point}$, $\ctime\geq0$, denotes the solution orbit of \eqref{eq:GD} starting at $\point$ at time $\ctime=0$.}
We then have the following notion of ``asymptotic closeness'':
%due to \citet{BH96}:

%\NH{Note that trajectories and orbit entities were not defined, which to the unfamiliar reader might be unclear. However, I am not sure you need to do anything about it. You can also just ref to some book.}
%\PM{I see your concern;
%I dropped ``orbit'' but I otherwise left things as they are, if a reviewer doesn't understand this part, they won't be able to follow the rest of the paper eithe\dots}

\begin{definition}
\label{def:APT}
We say that $\apt{\ctime}$ is an \acdef{APT} of \eqref{eq:GD} if, for all $\horizon > 0$, we have:
\begin{equation}
\label{eq:APT}
\adjustlimits
\lim_{\ctime\to\infty}
	\sup_{0 \leq h \leq \horizon}
		\norm{\apt{\ctime + h} - \flow{h}{\apt{\ctime}}}
	= 0
\end{equation}
\end{definition}

This comparison criterion is due to \citet{BH96} and it plays a central role in the theory of \acl{SA}.
In plainer words, it simply posits that $\apt{\ctime}$ eventually tracks the flow of \eqref{eq:GD} with arbitrary accuracy over windows of arbitrary length.
When this is the case, we will slightly abuse terminology and say that the sequence $\curr$ itself comprises an \ac{APT} of \eqref{eq:GD}.

Thanks to the above, we are finally in a position to state the formal link between \eqref{eq:GD} and \eqref{eq:SGD}:
%precisely the fact that the iterates of \eqref{eq:SGD} comprise an \ac{APT} of \eqref{eq:GD}:

\begin{proposition}
\label{prop:APT}
Suppose that \cref{asm:reg,asm:noise} hold
and
\eqref{eq:SGD} is run with a variable step-size sequence such that $\sum_{\run=\start}^{\infty} \curr[\step] = \infty$ and $\sum_{\run=\start}^{\infty} \curr[\step]^{1+\qexp/2} < \infty$.
Then, with probability $1$, $\curr$ is an \ac{APT} of \eqref{eq:GD}.
\end{proposition}

\begin{corollary}
\label{cor:APT-step}
%Suppose that \cref{asm:reg,asm:noise} hold and \eqref{eq:SGD} is run with
Suppose that \cref{asm:reg,asm:noise} hold
and
\eqref{eq:SGD} is run with $\curr[\step]\propto 1/\run^{\pexp}$ for some $\pexp \in (2/(\qexp + 2),1]$.
Then, with probability $1$, $\curr$ is an \ac{APT} of \eqref{eq:GD}.
\end{corollary}

\Cref{prop:APT} follows from a tandem application of Propositions~4.1 and 4.2 in \citet{Ben99}, so we omit its proof.
\Cref{cor:APT-step} is key for the sequel because it sketches the class of admissible step-size policies for \ac{SGD};
all the step-size policies we consider will adhere to the above desiderata.

==> Stability.tex <==
%----------------------------------------------------------------------
%%% STABILITY
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


Heuristically, the benefit of approximating \eqref{eq:SGD} via \eqref{eq:GD} is to allow the strong convergence properties of the latter to descend to the former.
However, a crucial obstacle that arises in this context is that the limit set of an \ac{APT} and that of a continuous-time flow, can be \emph{completely} different;
for concreteness, we provide an example of this fundamental discrepancy
in the paper's supplement.
%to wit, in the paper's supplement, we provide a simple example of a planar flow all of whose orbits converge to the $x$-axis ($y=0$), but which admits as an \acl{APT} the line $y=1$.
%\NH{Last sentence is confusing}

Because of this disconnect, the notion of an \ac{APT} is \emph{not sufficient} in general to act as a conduit from continuous to discrete time by itself.
The principal reason for this failure is that \acp{APT} may escape to infinity, in which case the \acl{SA} becomes \emph{unstable} \citep{Ben99,Bor08}.
{Thus,} a common way to guarantee a ``stable approximation'' is to assume that the \acp{APT} are \emph{precompact}, \ie that
\begin{equation}
\label{eq:stability}
\txs
\sup_{\ctime\geq\cstart} \norm{\apt{\ctime}}
	< \infty
	\quad
	\as.
\end{equation}
%\NH{The introduction to precompactness feels to me too detailed, I suggest to omit the description of the example, and contract a bit on the intuitive explanation (did it, original in remark)}
%\PM{Is the current version ok for you?}

A major difficulty that arises here is that the boundedness condition \eqref{eq:stability} is \emph{implicit}, so it typically needs to be enforced ``by hand'', see \eg \citet[Chap.~2]{Bor08}.
Therefore, unless boundedness can be somehow certified ahead of time, any theoretical result relying on {precompactness}
%the stability of \eqref{eq:SGD} as a \acl{RM} scheme
would be of limited applicability to machine learning problems.

%In view of this, our first step will be to establish the following stability result for the \acp{APT} of the dynamics \eqref{eq:GD}:
Our first result below provides exactly this certification, and is therefore the key to unlocking the use of \acl{SA} results and techniques in the sequel:

\begin{restatable}{theorem}{stability}
\label{thm:stability}
Suppose that \crefrange{asm:reg}{asm:noise} hold
and
\eqref{eq:SGD} is run with a variable step-size sequence
of the form $\curr[\step]\propto 1/\run^{\pexp}$ for some $\pexp \in (2/(\qexp + 2),1]$.
%such that $\sum_{\run=\start}^{\infty} \curr[\step] = \infty$ and $\sum_{\run=\start}^{\infty} \curr[\step]^{1+\qexp/2} < \infty$.
Then, with probability $1$, every \ac{APT} $\apt{\ctime}$ of \eqref{eq:GD} that is induced by \eqref{eq:SGD} has $\sup_{\ctime\geq\cstart} \norm{\apt{\ctime}} < \infty$.
\end{restatable}

This theorem plays a major role in the rest of our paper.
{Because of the generality of our assumptions, the proof of \cref{thm:stability} is fairly arduous and non-standard.}
For this reason, we devote the rest of this section to sketching said proof via a series of intermediate results of independent value (for the details, we refer the reader to the paper's supplement).
%We do so via a series of intermediate results that are of independent interest.

The first is that \eqref{eq:SGD} admits a convergent subsequence:

\begin{restatable}{lemma}{subsequence}
\label{lem:subsequence}
With assumptions as in \cref{thm:stability}, there exists a \textpar{possibly random} subsequence $\state_{\run_{\runalt}}$ of $\curr$ that converges to $\sols$;
formally, $\liminf_{\run\to\infty} \dist(\curr,\sols) = 0$ \as.
\end{restatable}

The proof of \cref{lem:subsequence} relies on a series of probabilistic estimates and proceeds by contradiction.
Its main component is the recursive estimate
\begin{align}
\label{eq:energy}
\obj(\next)
	\leq \obj(\curr)
		- \curr[\step] \braket{\nabla\obj(\curr)}{\curr[\noise]}
		+ \frac{\smooth}{2} \curr[\step]^{2} \norm{\curr[\signal]}^{2}
%	\notag\\
		- \curr[\step] \norm{\nabla\obj(\curr)}^{2},
\end{align}
which is a consequence of the Lipschitz smoothness requirement \eqref{eq:Lip-smooth} and the definition of \eqref{eq:SGD}.
In particular, if $\curr$ stays a positive distance away from $\sols$, a topological argument combining \cref{asm:reg,asm:gradlvl} shows that the last term in \eqref{eq:energy} provides a $\Theta(\curr[\step])$ contribution to $\obj(\curr)$ at each step.
If the stochastic terms in \eqref{eq:SGD} were uniformly bounded, the summability conditions for $\curr[\step]$ would suffice to show directly that this $\Theta(\curr[\step])$ contribution dominates \eqref{eq:energy}, leading in turn to $\obj(\curr) \to -\infty$, a contradiction (by \cref{asm:sublvl}).
However, seeing as the noise is not bounded, we need to invoke instead a specialized version of the law of large numbers for \aclp{MDS} as well as Doob's submartingale convergence theorem \citep{HH80} to conclude that this contradiction still occurs under the more general noise hypotheses stated in \cref{asm:noise}.
We defer the numerous subtleties of this argument to the paper's supplement.

%That being said, we should note here that this result is conceptually quite important because it states that $\curr$ returns arbitrarily close to $\sols$ infinitely often.
%Intuitively, this means that $\curr$ has an infinite number of chances to be captured by $\sols$, so it is a key stepping stone towards proving that this ``entrapment'' actually occurs.

Moving forward, our second result is more technical in nature and provides a deeper look into the function minimization properties of the continuous-time dynamics \eqref{eq:GD}.
Heuristically, it states that the trajectories of \eqref{eq:GD} either descend the objective function by a uniform amount, or they have already reached a certain neighborhood of $\sols$.

To state this result precisely, let
\begin{equation}
\label{eq:critval}
\critval
	= \max\nolimits_{\point\in\sols} \obj(\point)
\end{equation}
denote the maximal value of $\obj$ over its critical set,%
\footnote{That $\critval$ exists and is finite is a consequence of the fact that $\sols$ is compact;
\cf the discussion in \cref{sec:setup}.}
and let
\begin{equation}
\label{eq:critnhd}
\critnhd_{\eps}
	\equiv \flvl_{\critval + \eps}
	= \setdef{\point\in\points}{\obj(\point) \leq \critval + \eps}
\end{equation}
denote the $(\critval + \eps)$-sublevel set of $\eps\geq0$.
We then have the following formal statement:
%\NH{Moved footnote place to end of sentence, I think this is the rule in English (you may disagree).}
%\PM{The rule is after the punctuation if any punctuation there is, so I moved it right after the comma (where it is more appropriate).}
\begin{restatable}{lemma}{decrease}
\label{lem:decrease}
Fix some $\eps>0$.
Under \cref{asm:reg,asm:sublvl,asm:gradlvl}, there exists some $\tau \equiv \tau(\eps)$ such that, for all $\point\in\points$, we have
\begin{enumerate*}
[\upshape(\itshape i\hspace*{.5pt}\upshape)]
\item
$\obj(\flow{\tau}{\point}) \leq \obj(\point) - \eps$;
or
\item
$\flow{\tau}{\point} \in \critnhd_{\eps}$.
\end{enumerate*}
\end{restatable}

The proof of \cref{lem:decrease} relies on a stopping time estimate and a localized LaSalle invariance argument;
we defer all details to the supplement.

Finally, the last technical result that we will need is a value comparison criterion between solution trajectories of \eqref{eq:GD} and \aclp{APT} thereof.

\begin{restatable}{lemma}{flowAPT}
\label{lem:flowAPT}
Fix some $\eps,\delta>0$.
Then, with assumptions and notation as in \cref{lem:decrease}, there exists some $\ctime_{0} \equiv \ctime_{0}(\delta,\eps)$ such that, for all $\ctime \geq \ctime_{0}$ and all $h \in [0,\tau]$, we have:
\begin{equation}
\label{eq:flowAPT}
\obj(\apt{\ctime + h})
	\leq \obj(\flow{h}{\apt{\ctime}})
		+ \lips \delta
		+ \tfrac{1}{2} \smooth \delta^{2}.
\end{equation}
\end{restatable}
In words, \cref{lem:flowAPT} states that, asymptotically, the evolution of $\obj$ under an \ac{APT} $\apt{\ctime}$ can be approximated by its evolution under \eqref{eq:GD} up to a uniformly small error.
%\NH{the notion of drift was not defined, which makes this statement confusing (at least for me)}
%\PM{Better now?}
This result relies on \cref{lem:decrease} and the regularity properties of $\obj$,
and is the last ingredient we need for the proof of \cref{thm:stability}.
The technical chassis of the argument (which we make precise in the supplement) proceeds as follows:

\begin{proof}[Sketch of proof of \cref{thm:stability}]
\hfill
\begin{enumerate}
\item
First, \cref{lem:subsequence} guarantees that $\apt{\ctime}$ eventually comes arbitrarily close to $\sols$;
specifically, there exists some $\ctime_{1} > 0$ such that $\apt{\ctime_{1}} \in \critnhd_{2\eps}$.

\item
By \cref{lem:flowAPT}, there exists some uniform time window $\tau$ such that $\apt{\ctime}$ remains close to $\critnhd_{2\eps}$ within this window;
more precisely, we have $\apt{\ctime} \in \critnhd_{3\eps}$ for all $\ctime \in [\ctime_{1},\ctime_{1} + \tau]$.

\item
By putting \cref{lem:decrease,lem:flowAPT} together, we further conclude that $\apt{\ctime_{1} + \tau} \in \critnhd_{2\eps}$ at the end of said window.

\item
Since $\apt{\ctime_{1}},\apt{\ctime_{1}+\tau} \in \critnhd_{2\eps}$ and $\apt{\ctime} \in \critnhd_{3\eps}$ for all $\ctime\in[\ctime_{1},\ctime_{1} + \tau]$, we may iterate the above argument to show inductively that the same holds over all intervals of the form $[\ctime_{1} + \runalt\tau, \ctime_{1} + (\runalt+1)\tau]$.
\end{enumerate}

Since $\critnhd_{3\eps} = \flvl_{\critval + 3\eps}$ is bounded (by \cref{asm:sublvl}), we conclude that $\apt{\ctime}$ remains in a compact set for all $\ctime\geq0$, \ie $\apt{\ctime}$ is precompact.
\Cref{thm:stability} then follows by noting that, under the stated step-size assumptions, any affine interpolation of $\curr$ is an \ac{APT} of \eqref{eq:GD}.
\end{proof}
